Estimation of the Number of Components of Non-Parametric Multivariate Finite Mixture Models

We propose a novel estimator for the number of components (denoted by $M$) in a K-variate non-parametric finite mixture model, where the analyst has repeated observations of $K\geq2$ variables that are independent given a finitely supported unobserved variable. Under a mild assumption on the joint distribution of the observed and latent variables, we show that an integral operator $T$, that is identified from the data, has rank equal to $M$. Using this observation, and the fact that singular values are stable under perturbations, the estimator of $M$ that we propose is based on a thresholding rule which essentially counts the number of singular values of a consistent estimator of $T$ that are greater than a data-driven threshold. We prove that our estimator of $M$ is consistent, and establish non-asymptotic results which provide finite sample performance guarantees for our estimator. We present a Monte Carlo study which shows that our estimator performs well for samples of moderate size.

==> 3_normal.tex <==
\begin{tabular}{cc|cccc|cccc}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M\geq 4$ & $M=1$ & $M=2$ & $M=3$ & $M\geq 4$ \tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} & 1.000 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000\tabularnewline
\hline
$M_{0}=4$ & SHT & 0.021 & 0.891 & 0.082 & 0.006 & 0.000 & 0.566 & 0.414 & 0.020\tabularnewline
 & AIC & 0.004 & 0.757 & 0.215 & 0.024 & 0.000 & 0.317 & 0.609 & 0.074\tabularnewline
 & BIC & 0.464 & 0.533 & 0.003 & 0.000 & 0.000 & 0.989 & 0.011 & 0.000\tabularnewline
 & HQ & 0.092 & 0.876 & 0.031 & 0.001 & 0.000 & 0.766 & 0.226 & 0.008\tabularnewline
 \hline
$M_{0}=8$ & SHT & 0.094 & 0.874 & 0.032 & 0.000 & 0.000 & 0.690 & 0.306 & 0.004\tabularnewline
 & AIC & 0.022 & 0.830 & 0.148 & 0.000 & 0.000 & 0.384 & 0.542 & 0.074\tabularnewline
 & BIC & 0.704 & 0.296 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000\tabularnewline
 & HQ & 0.212 & 0.788 & 0.000 & 0.000 & 0.000 & 0.954 & 0.046 & 0.000\tabularnewline
 \hline

\end{tabular}



==> 3_normal_new.tex <==
\begin{tabular}{cc|cccc|cccc}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M\geq4$ & $M=1$ & $M=2$ & $M=3$ & $M\geq4$\tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} & 0.072 &  0.928 & 0.000 &  0.000& 0.000 & 0.000 & 1.000 &0.000 \tabularnewline
\hline
$M_{0}=4$ & SHT & 0.000 & 0.000 & 0.980 & 0.020 & 0.000 & 0.000 & 0.950 & 0.050\tabularnewline
 & AIC & 0.000 & 0.000 & 0.886 & 0.114 & 0.000 & 0.000 & 0.882 & 0.118\tabularnewline
 & BIC & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.992 & 0.008\tabularnewline
 & HQ & 0.000 & 0.000 & 0.978 & 0.022 & 0.000 & 0.000 & 0.958 & 0.042\tabularnewline
 \hline
$M_{0}=8$ & SHT & 0.000 & 0.000 & 0.940 & 0.060 & 0.000 & 0.000 & 0.930 & 0.070\tabularnewline
 & AIC & 0.000 & 0.000 & 0.824 & 0.176 & 0.000 & 0.000 & 0.806 & 0.194\tabularnewline
 & BIC & 0.000 & 0.000 & 0.992 & 0.008 & 0.000 & 0.000 & 0.998 & 0.002\tabularnewline
 & HQ & 0.000 & 0.000 & 0.964 & 0.036 & 0.000 & 0.000 & 0.968 & 0.032\tabularnewline
\hline
\end{tabular}


==> 3_uniform.tex <==
\begin{tabular}{cc|cccc|cccc}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M\geq4$ & $M=1$ & $M=2$ & $M=3$ & $M\geq4$\tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} & 0.000 & 0.002 & 0.996 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000\tabularnewline
\hline
$M_{0}=4$ & SHT  & 0.425 & 0.000 & 0.575 & 0.000 & 0.520 & 0.000 & 0.480 & 0.000\tabularnewline
 & AIC & 0.454 & 0.000 & 0.544 & 0.002 & 0.452 & 0.000 & 0.492 & 0.056\tabularnewline
 & BIC & 0.410 & 0.000 & 0.590 & 0.000 & 0.497 & 0.000 & 0.458 & 0.045\tabularnewline
 & HQ & 0.422 & 0.000 & 0.578 & 0.000 & 0.520 & 0.000 & 0.462 & 0.018\tabularnewline
 \hline
$M_{0}=8$ & SHT & 0.382 & 0.013 & 0.072 & 0.523 & 0.478 & 0.244 & 0.002 & 0.276\tabularnewline
 & AIC & 0.362 & 0.018 & 0.028 & 0.592 & 0.466 & 0.204 & 0.000 & 0.330\tabularnewline
 & BIC & 0.339 & 0.028 & 0.140 & 0.493 & 0.472 & 0.224 & 0.004 & 0.300\tabularnewline
 & HQ & 0.352 & 0.018 & 0.076 & 0.554 & 0.476 & 0.282 & 0.000 & 0.242\tabularnewline
\hline
\end{tabular}



==> 5_uniform.tex <==
\begin{tabular}{cc|cccccc|cccccc}
 & \multicolumn{1}{c}{} & \multicolumn{6}{c}{$N=500$} & \multicolumn{6}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M=4$ & $M=5$ & $M\geq 5$ & $M=1$ & $M=2$ & $M=3$ & $M=4$ & $M=5$ & $M\geq 5$\tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} &0.000  & 0.000 &  0.992&  0.008& 0.000&  0.000&  0.000&  0.000&  0.000 &0.000& 1.000 & 0.000  \tabularnewline
\hline
$M_{0}=4$ & SHT & 0.466 & 0.000 & 0.000 & 0.534 &0.000& 0.000 & 0.484 & 0.000 & 0.000 & 0.516& 0.000 & 0.000 \tabularnewline
 & AIC & 0.475 & 0.000 & 0.000 & 0.525 &0.000& 0.000&0.478 & 0.000 & 0.000 & 0.522&0.000&0.000\tabularnewline
 & BIC & 0.481 & 0.000 & 0.000 & 0.519 &0.000&0.000& 0.470 & 0.000 & 0.000 & 0.530&0.000&0.000\tabularnewline
 & HQ & 0.480 & 0.000 & 0.000 & 0.520 &0.000&0.000&  0.482 & 0.000 & 0.000 & 0.518&0.000&0.000\tabularnewline
  \hline
$M_{0}=8$ & SHT & 0.458 & 0.208 & 0.013 & 0.170 &0.083&0.068&  0.504 & 0.274 & 0.000 & 0.072&0.097&0.053\tabularnewline
 & AIC & 0.430 & 0.212 & 0.014 & 0.213 &0.075&0.056&  0.458 & 0.328 & 0.000 & 0.078 &0.089&0.047\tabularnewline
 & BIC & 0.415 & 0.225 & 0.019 & 0.227 &0.067&0.047&  0.449 & 0.325 & 0.000 & 0.109&0.086&0.031\tabularnewline
 & HQ & 0.422 & 0.216 & 0.022 & 0.216 &0.081&0.043&  0.461 & 0.324 & 0.000 & 0.093&0.094&0.028\tabularnewline
\hline
\end{tabular}



==> Tables/design5.tex <==
\begin{tabular}{cc|cccc|cccc}
\hline 
 & \multicolumn{1}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{Method} & $M=1$ & $M=2$ & $M=3$ & $M\protect\geq4$ & $M=1$ & $M=2$ & $M=3$ & $M\protect\geq4$\tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} & 0.000 & 0.992 & 0.008 & 0.000 & 0.000 & 0.493 & 0.507 & 0.000\tabularnewline
\hline 
\multicolumn{2}{c|}{ave-rk $(\alpha=0.05)$} & 0.142 & 0.810 & 0.047 & 0.001 & 0.005 & 0.776 & 0.214 & 0.005\tabularnewline
\multicolumn{2}{c|}{AIC by ave-rk} & 0.012 & 0.867 & 0.119 & 0.003 & 0.000 & 0.587 & 0.399 & 0.013\tabularnewline
\multicolumn{2}{c|}{BIC by ave-rk} & 0.284 & 0.715 & 0.001 & 0.000 & 0.035 & 0.942 & 0.023 & 0.000\tabularnewline
\multicolumn{2}{c|}{HQ by ave-rk} & 0.078 & 0.909 & 0.013 & 0.000 & 0.004 & 0.878 & 0.117 & 0.001\tabularnewline
\end{tabular}



==> Tables/design7.tex <==
\begin{tabular}{cc|cccc|cccc}
 & \multicolumn{1}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M\geq 4$ & $M=1$ & $M=2$ & $M=3$ & $M\geq 4$ \tabularnewline
\hline 
\multicolumn{2}{c|}{SVT} & 1.000 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000\tabularnewline
\hline
$M_{0}=4$ & SHT & 0.021 & 0.891 & 0.082 & 0.006 & 0.000 & 0.566 & 0.414 & 0.020\tabularnewline
 & AIC & 0.004 & 0.757 & 0.215 & 0.024 & 0.000 & 0.317 & 0.609 & 0.074\tabularnewline
 & BIC & 0.464 & 0.533 & 0.003 & 0.000 & 0.000 & 0.989 & 0.011 & 0.000\tabularnewline
 & HQ & 0.092 & 0.876 & 0.031 & 0.001 & 0.000 & 0.766 & 0.226 & 0.008\tabularnewline
 \hline
$M_{0}=8$ & SHT & 0.094 & 0.874 & 0.032 & 0.000 & 0.000 & 0.690 & 0.306 & 0.004\tabularnewline
 & AIC & 0.022 & 0.830 & 0.148 & 0.000 & 0.000 & 0.384 & 0.542 & 0.074\tabularnewline
 & BIC & 0.704 & 0.296 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000 & 0.000\tabularnewline
 & HQ & 0.212 & 0.788 & 0.000 & 0.000 & 0.000 & 0.954 & 0.046 & 0.000\tabularnewline
 \hline

\end{tabular}



==> Tables/design7_-_Copy.tex <==
\begin{tabular}{c||c|cccc|cccc}
\multicolumn{2}{c}{} & \multicolumn{4}{c}{$N=500$} & \multicolumn{4}{c}{$N=2000$}\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M=1$ & $M=2$ & $M=3$ & $M\protect\geq4$ & $M=1$ & $M=2$ & $M=3$ & $M\protect\geq4$\tabularnewline
\hline 
\multicolumn{2}{c|}{Design 1} & 0.001 & 0.893 & 0.106 & 0.000 & 0.000 & 0.179 & 0.818 & 0.003\tabularnewline
\multicolumn{2}{c|}{Design 2} & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.972 & 0.028\tabularnewline
\multicolumn{2}{c|}{Design 3} & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000 & 0.999 & 0.001\tabularnewline
\multicolumn{2}{c|}{Design 5} & 0.000 & 0.781 & 0.219 & 0.000 & 0.000 & 0.000 & 0.985 & 0.015\tabularnewline
\hline 
\multicolumn{2}{c|}{} & $M\protect\leq3$ & $M=4$ & $M=5$ & $M=6$ & $M\protect\leq3$ & $M=4$ & $M=5$ & $M=6$\tabularnewline
\hline 
\multicolumn{2}{c|}{Design 4} & 0.000 & 0.000 & 1.000 & 0.000 & 0.000 & 0.000 & 1.000 & 0.000\tabularnewline
\end{tabular}}


